Strictly Frequentist Imprecise Probability

Strict frequentism defines probability as the limiting relative frequency in an infinite sequence. What if the limit does not exist? We present a broader theory, which is applicable also to random phenomena that exhibit diverging relative frequencies. In doing so, we develop a close connection with the theory of imprecise probability: the cluster points of relative frequencies yield a coherent upper prevision. We show that a natural frequentist definition of conditional probability recovers the generalized Bayes rule. This also suggests an independence concept, which is related to epistemic irrelevance in the imprecise probability literature. Finally, we prove constructively that, for a finite set of elementary events, there exists a sequence for which the cluster points of relative frequencies coincide with a prespecified set which demonstrates the naturalness, and arguably completeness, of our theory.

==> figures/drawing.tex <==
%LaTeX with PSTricks extensions
%%Creator: Inkscape 1.2.1 (9c6d41e, 2022-07-14)
%%Please note this file requires PSTricks extensions
\psset{xunit=.5pt,yunit=.5pt,runit=.5pt}
\begin{pspicture}(793.7007874,1122.51968504)
{
\newrgbcolor{curcolor}{0.96470588 1 0.83529413}
\pscustom[linestyle=none,fillstyle=solid,fillcolor=curcolor]
{
\newpath
\moveto(39.41911856,388.90259454)
\lineto(383.59047656,999.00110121)
\lineto(730.51888357,390.52303298)
\closepath
}
}
{
\newrgbcolor{curcolor}{0.03529412 0 0.03137255}
\pscustom[linewidth=1.88791529,linecolor=curcolor]
{
\newpath
\moveto(39.41911856,388.90259454)
\lineto(383.59047656,999.00110121)
\lineto(730.51888357,390.52303298)
\closepath
}
}
{
\newrgbcolor{curcolor}{0.03529412 0 0.03137255}
\pscustom[linewidth=1.15850073,linecolor=curcolor]
{
\newpath
\moveto(545.09476033,533.77371704)
\lineto(404.36560127,415.46498003)
\lineto(247.72065135,488.89798791)
\lineto(316.68090206,654.90802885)
\lineto(452.95067214,687.16712806)
\closepath
}
}
{
\newrgbcolor{curcolor}{0 0 0}
\pscustom[linestyle=none,fillstyle=solid,fillcolor=curcolor]
{
\newpath
\moveto(318.90513346,664.66804744)
\curveto(318.90513346,662.91068807)(317.55965796,661.48606683)(315.89992982,661.48606683)
\curveto(314.24020168,661.48606683)(312.89472618,662.91068807)(312.89472618,664.66804744)
\curveto(312.89472618,666.42540681)(314.24020168,667.85002805)(315.89992982,667.85002805)
\curveto(317.55965796,667.85002805)(318.90513346,666.42540681)(318.90513346,664.66804744)
\closepath
}
}
{
\newrgbcolor{curcolor}{0.03529412 0 0.03137255}
\pscustom[linewidth=0.99999871,linecolor=curcolor]
{
\newpath
\moveto(318.90513346,664.66804744)
\curveto(318.90513346,662.91068807)(317.55965796,661.48606683)(315.89992982,661.48606683)
\curveto(314.24020168,661.48606683)(312.89472618,662.91068807)(312.89472618,664.66804744)
\curveto(312.89472618,666.42540681)(314.24020168,667.85002805)(315.89992982,667.85002805)
\curveto(317.55965796,667.85002805)(318.90513346,666.42540681)(318.90513346,664.66804744)
\closepath
}
}
{
\newrgbcolor{curcolor}{0 0 0}
\pscustom[linestyle=none,fillstyle=solid,fillcolor=curcolor]
{
\newpath
\moveto(455.55357288,686.23484393)
\curveto(455.55357288,684.47748456)(454.20809738,683.05286332)(452.54836924,683.05286332)
\curveto(450.8886411,683.05286332)(449.5431656,684.47748456)(449.5431656,686.23484393)
\curveto(449.5431656,687.9922033)(450.8886411,689.41682454)(452.54836924,689.41682454)
\curveto(454.20809738,689.41682454)(455.55357288,687.9922033)(455.55357288,686.23484393)
\closepath
}
}
{
\newrgbcolor{curcolor}{0.03529412 0 0.03137255}
\pscustom[linewidth=0.99999871,linecolor=curcolor]
{
\newpath
\moveto(455.55357288,686.23484393)
\curveto(455.55357288,684.47748456)(454.20809738,683.05286332)(452.54836924,683.05286332)
\curveto(450.8886411,683.05286332)(449.5431656,684.47748456)(449.5431656,686.23484393)
\curveto(449.5431656,687.9922033)(450.8886411,689.41682454)(452.54836924,689.41682454)
\curveto(454.20809738,689.41682454)(455.55357288,687.9922033)(455.55357288,686.23484393)
\closepath
}
}
{
\newrgbcolor{curcolor}{0 0 0}
\pscustom[linestyle=none,fillstyle=solid,fillcolor=curcolor]
{
\newpath
\moveto(456.59952322,708.22007246)
\curveto(456.59952322,706.4627131)(455.25404772,705.03809185)(453.59431958,705.03809185)
\curveto(451.93459144,705.03809185)(450.58911595,706.4627131)(450.58911595,708.22007246)
\curveto(450.58911595,709.97743183)(451.93459144,711.40205308)(453.59431958,711.40205308)
\curveto(455.25404772,711.40205308)(456.59952322,709.97743183)(456.59952322,708.22007246)
\closepath
}
}
{
\newrgbcolor{curcolor}{0.03529412 0 0.03137255}
\pscustom[linewidth=0.99999871,linecolor=curcolor]
{
\newpath
\moveto(456.59952322,708.22007246)
\curveto(456.59952322,706.4627131)(455.25404772,705.03809185)(453.59431958,705.03809185)
\curveto(451.93459144,705.03809185)(450.58911595,706.4627131)(450.58911595,708.22007246)
\curveto(450.58911595,709.97743183)(451.93459144,711.40205308)(453.59431958,711.40205308)
\curveto(455.25404772,711.40205308)(456.59952322,709.97743183)(456.59952322,708.22007246)
\closepath
}
}
{
\newrgbcolor{curcolor}{0 0 0}
\pscustom[linestyle=none,fillstyle=solid,fillcolor=curcolor]
{
\newpath
\moveto(555.25556753,701.79116737)
\curveto(555.25556753,700.033808)(553.91009203,698.60918675)(552.25036389,698.60918675)
\curveto(550.59063575,698.60918675)(549.24516025,700.033808)(549.24516025,701.79116737)
\curveto(549.24516025,703.54852673)(550.59063575,704.97314798)(552.25036389,704.97314798)
\curveto(553.91009203,704.97314798)(555.25556753,703.54852673)(555.25556753,701.79116737)
\closepath
}
}
{
\newrgbcolor{curcolor}{0.03529412 0 0.03137255}
\pscustom[linewidth=0.99999871,linecolor=curcolor]
{
\newpath
\moveto(555.25556753,701.79116737)
\curveto(555.25556753,700.033808)(553.91009203,698.60918675)(552.25036389,698.60918675)
\curveto(550.59063575,698.60918675)(549.24516025,700.033808)(549.24516025,701.79116737)
\curveto(549.24516025,703.54852673)(550.59063575,704.97314798)(552.25036389,704.97314798)
\curveto(553.91009203,704.97314798)(555.25556753,703.54852673)(555.25556753,701.79116737)
\closepath
}
}
{
\newrgbcolor{curcolor}{0 0 0}
\pscustom[linestyle=none,fillstyle=solid,fillcolor=curcolor]
{
\newpath
\moveto(536.19495145,733.69927053)
\curveto(536.19495145,731.94191116)(534.84947595,730.51728991)(533.18974781,730.51728991)
\curveto(531.53001967,730.51728991)(530.18454417,731.94191116)(530.18454417,733.69927053)
\curveto(530.18454417,735.45662989)(531.53001967,736.88125114)(533.18974781,736.88125114)
\curveto(534.84947595,736.88125114)(536.19495145,735.45662989)(536.19495145,733.69927053)
\closepath
}
}
{
\newrgbcolor{curcolor}{0.03529412 0 0.03137255}
\pscustom[linewidth=0.99999871,linecolor=curcolor]
{
\newpath
\moveto(536.19495145,733.69927053)
\curveto(536.19495145,731.94191116)(534.84947595,730.51728991)(533.18974781,730.51728991)
\curveto(531.53001967,730.51728991)(530.18454417,731.94191116)(530.18454417,733.69927053)
\curveto(530.18454417,735.45662989)(531.53001967,736.88125114)(533.18974781,736.88125114)
\curveto(534.84947595,736.88125114)(536.19495145,735.45662989)(536.19495145,733.69927053)
\closepath
}
}
{
\newrgbcolor{curcolor}{1 0 0}
\pscustom[linestyle=none,fillstyle=solid,fillcolor=curcolor]
{
\newpath
\moveto(315.36962143,665.02159106)
\lineto(552.25038867,701.79114066)
\lineto(551.89700285,702.49825247)
}
}
{
\newrgbcolor{curcolor}{1 0.16862746 0.16862746}
\pscustom[linewidth=0.99999871,linecolor=curcolor]
{
\newpath
\moveto(315.36962143,665.02159106)
\lineto(552.25038867,701.79114066)
\lineto(551.89700285,702.49825247)
}
}
{
\newrgbcolor{curcolor}{1 0 0}
\pscustom[linestyle=none,fillstyle=solid,fillcolor=curcolor]
{
\newpath
\moveto(431.20712568,932.56994003)
\lineto(417.70706899,924.56994255)
\lineto(417.70706899,924.56994255)
}
}
{
\newrgbcolor{curcolor}{0.16862746 0.19215687 1}
\pscustom[linewidth=0.99999871,linecolor=curcolor]
{
\newpath
\moveto(431.20712568,932.56994003)
\lineto(417.70706899,924.56994255)
\lineto(417.70706899,924.56994255)
}
}
{
\newrgbcolor{curcolor}{1 0 0}
\pscustom[linestyle=none,fillstyle=solid,fillcolor=curcolor]
{
\newpath
\moveto(466.95710993,870.06993373)
\lineto(453.45709104,862.06993625)
\lineto(453.45709104,862.06993625)
}
}
{
\newrgbcolor{curcolor}{0.16862746 0.19215687 1}
\pscustom[linewidth=0.99999871,linecolor=curcolor]
{
\newpath
\moveto(466.95710993,870.06993373)
\lineto(453.45709104,862.06993625)
\lineto(453.45709104,862.06993625)
}
}
{
\newrgbcolor{curcolor}{1 0 0}
\pscustom[linestyle=none,fillstyle=solid,fillcolor=curcolor]
{
\newpath
\moveto(501.95712253,804.56993877)
\lineto(488.45710363,796.56994129)
\lineto(488.45710363,796.56994129)
}
}
{
\newrgbcolor{curcolor}{0.16862746 0.19215687 1}
\pscustom[linewidth=0.99999871,linecolor=curcolor]
{
\newpath
\moveto(501.95712253,804.56993877)
\lineto(488.45710363,796.56994129)
\lineto(488.45710363,796.56994129)
}
}
{
\newrgbcolor{curcolor}{1 0 0}
\pscustom[linestyle=none,fillstyle=solid,fillcolor=curcolor]
{
\newpath
\moveto(539.95709734,737.56992491)
\lineto(526.45707844,729.56995011)
\lineto(526.45707844,729.56995011)
}
}
{
\newrgbcolor{curcolor}{0.16862746 0.19215687 1}
\pscustom[linewidth=0.99999871,linecolor=curcolor]
{
\newpath
\moveto(539.95709734,737.56992491)
\lineto(526.45707844,729.56995011)
\lineto(526.45707844,729.56995011)
}
}
{
\newrgbcolor{curcolor}{1 0 0}
\pscustom[linestyle=none,fillstyle=solid,fillcolor=curcolor]
{
\newpath
\moveto(582.95712253,663.06991861)
\lineto(569.45710363,655.06994381)
\lineto(569.45710363,655.06994381)
}
}
{
\newrgbcolor{curcolor}{0.16862746 0.19215687 1}
\pscustom[linewidth=0.99999871,linecolor=curcolor]
{
\newpath
\moveto(582.95712253,663.06991861)
\lineto(569.45710363,655.06994381)
\lineto(569.45710363,655.06994381)
}
}
{
\newrgbcolor{curcolor}{1 0 0}
\pscustom[linestyle=none,fillstyle=solid,fillcolor=curcolor]
{
\newpath
\moveto(617.95709734,601.06994381)
\lineto(604.45707844,593.06993121)
\lineto(604.45707844,593.06993121)
}
}
{
\newrgbcolor{curcolor}{0.16862746 0.19215687 1}
\pscustom[linewidth=0.99999871,linecolor=curcolor]
{
\newpath
\moveto(617.95709734,601.06994381)
\lineto(604.45707844,593.06993121)
\lineto(604.45707844,593.06993121)
}
}
{
\newrgbcolor{curcolor}{1 0 0}
\pscustom[linestyle=none,fillstyle=solid,fillcolor=curcolor]
{
\newpath
\moveto(652.95710993,540.06995641)
\lineto(639.45709104,532.06994381)
\lineto(639.45709104,532.06994381)
}
}
{
\newrgbcolor{curcolor}{0.16862746 0.19215687 1}
\pscustom[linewidth=0.99999871,linecolor=curcolor]
{
\newpath
\moveto(652.95710993,540.06995641)
\lineto(639.45709104,532.06994381)
\lineto(639.45709104,532.06994381)
}
}
{
\newrgbcolor{curcolor}{1 0 0}
\pscustom[linestyle=none,fillstyle=solid,fillcolor=curcolor]
{
\newpath
\moveto(693.95712253,469.06990602)
\lineto(680.45710363,461.06993121)
\lineto(680.45710363,461.06993121)
}
}
{
\newrgbcolor{curcolor}{0.16862746 0.19215687 1}
\pscustom[linewidth=0.99999871,linecolor=curcolor]
{
\newpath
\moveto(693.95712253,469.06990602)
\lineto(680.45710363,461.06993121)
\lineto(680.45710363,461.06993121)
}
}
{
\newrgbcolor{curcolor}{1 0 0}
\pscustom[linestyle=none,fillstyle=solid,fillcolor=curcolor]
{
\newpath
\moveto(316.70710174,665.06993121)
\lineto(534.70710678,734.06993121)
\lineto(534.20711308,734.06993121)
}
}
{
\newrgbcolor{curcolor}{0.16862746 0.19215687 1}
\pscustom[linewidth=0.99999871,linecolor=curcolor]
{
\newpath
\moveto(316.70710174,665.06993121)
\lineto(534.70710678,734.06993121)
\lineto(534.20711308,734.06993121)
}
}
{
\newrgbcolor{curcolor}{1 0 0}
\pscustom[linestyle=none,fillstyle=solid,fillcolor=curcolor]
{
\newpath
\moveto(406.0373619,689.52320995)
\lineto(403.90037923,696.468432)
}
}
{
\newrgbcolor{curcolor}{0.98823529 0.10980392 0.98039216}
\pscustom[linewidth=0.99999871,linecolor=curcolor]
{
\newpath
\moveto(406.0373619,689.52320995)
\lineto(403.90037923,696.468432)
}
}
{
\newrgbcolor{curcolor}{1 0 0}
\pscustom[linestyle=none,fillstyle=solid,fillcolor=curcolor]
{
\newpath
\moveto(422.65919497,694.62307767)
\lineto(420.5222123,701.56829972)
}
}
{
\newrgbcolor{curcolor}{0.98823529 0.10980392 0.98039216}
\pscustom[linewidth=0.99999871,linecolor=curcolor]
{
\newpath
\moveto(422.65919497,694.62307767)
\lineto(420.5222123,701.56829972)
}
}
{
\newrgbcolor{curcolor}{1 0 0}
\pscustom[linestyle=none,fillstyle=solid,fillcolor=curcolor]
{
\newpath
\moveto(437.95887371,699.53408239)
\lineto(435.82189104,706.47930444)
}
}
{
\newrgbcolor{curcolor}{0.98823529 0.10980392 0.98039216}
\pscustom[linewidth=0.99999871,linecolor=curcolor]
{
\newpath
\moveto(437.95887371,699.53408239)
\lineto(435.82189104,706.47930444)
}
}
{
\newrgbcolor{curcolor}{1 0 0}
\pscustom[linestyle=none,fillstyle=solid,fillcolor=curcolor]
{
\newpath
\moveto(454.95850836,704.63398791)
\lineto(452.82152568,711.57920995)
}
}
{
\newrgbcolor{curcolor}{0.98823529 0.10980392 0.98039216}
\pscustom[linewidth=0.99999871,linecolor=curcolor]
{
\newpath
\moveto(454.95850836,704.63398791)
\lineto(452.82152568,711.57920995)
}
}
{
\newrgbcolor{curcolor}{1 0 0}
\pscustom[linestyle=none,fillstyle=solid,fillcolor=curcolor]
{
\newpath
\moveto(470.44705009,710.1116194)
\lineto(468.31006741,717.05684145)
}
}
{
\newrgbcolor{curcolor}{0.98823529 0.10980392 0.98039216}
\pscustom[linewidth=0.99999871,linecolor=curcolor]
{
\newpath
\moveto(470.44705009,710.1116194)
\lineto(468.31006741,717.05684145)
}
}
{
\newrgbcolor{curcolor}{1 0 0}
\pscustom[linestyle=none,fillstyle=solid,fillcolor=curcolor]
{
\newpath
\moveto(487.63554773,715.21152491)
\lineto(485.49856505,722.15674696)
}
}
{
\newrgbcolor{curcolor}{0.98823529 0.10980392 0.98039216}
\pscustom[linewidth=0.99999871,linecolor=curcolor]
{
\newpath
\moveto(487.63554773,715.21152491)
\lineto(485.49856505,722.15674696)
}
}
{
\newrgbcolor{curcolor}{1 0 0}
\pscustom[linestyle=none,fillstyle=solid,fillcolor=curcolor]
{
\newpath
\moveto(504.63518237,721.25582098)
\lineto(502.4981997,728.20104302)
}
}
{
\newrgbcolor{curcolor}{0.98823529 0.10980392 0.98039216}
\pscustom[linewidth=0.99999871,linecolor=curcolor]
{
\newpath
\moveto(504.63518237,721.25582098)
\lineto(502.4981997,728.20104302)
}
}
{
\newrgbcolor{curcolor}{1 0 0}
\pscustom[linestyle=none,fillstyle=solid,fillcolor=curcolor]
{
\newpath
\moveto(519.93486111,725.41129814)
\lineto(517.79784064,732.35652019)
}
}
{
\newrgbcolor{curcolor}{0.98823529 0.10980392 0.98039216}
\pscustom[linewidth=0.99999871,linecolor=curcolor]
{
\newpath
\moveto(519.93486111,725.41129814)
\lineto(517.79784064,732.35652019)
}
}
{
\newrgbcolor{curcolor}{1 0 0}
\pscustom[linestyle=none,fillstyle=solid,fillcolor=curcolor]
{
\newpath
\moveto(337.93787592,668.51738948)
\lineto(335.80088946,675.46261153)
}
}
{
\newrgbcolor{curcolor}{0.98823529 0.10980392 0.98039216}
\pscustom[linewidth=0.99999871,linecolor=curcolor]
{
\newpath
\moveto(337.93787592,668.51738948)
\lineto(335.80088946,675.46261153)
}
}
{
\newrgbcolor{curcolor}{1 0 0}
\pscustom[linestyle=none,fillstyle=solid,fillcolor=curcolor]
{
\newpath
\moveto(356.1717871,674.412432)
\lineto(354.03480064,681.35765405)
}
}
{
\newrgbcolor{curcolor}{0.98823529 0.10980392 0.98039216}
\pscustom[linewidth=0.99999871,linecolor=curcolor]
{
\newpath
\moveto(356.1717871,674.412432)
\lineto(354.03480064,681.35765405)
}
}
{
\newrgbcolor{curcolor}{1 0 0}
\pscustom[linestyle=none,fillstyle=solid,fillcolor=curcolor]
{
\newpath
\moveto(373.73806363,679.8900635)
\lineto(371.60107718,686.83528554)
}
}
{
\newrgbcolor{curcolor}{0.98823529 0.10980392 0.98039216}
\pscustom[linewidth=0.99999871,linecolor=curcolor]
{
\newpath
\moveto(373.73806363,679.8900635)
\lineto(371.60107718,686.83528554)
}
}
{
\newrgbcolor{curcolor}{1 0 0}
\pscustom[linestyle=none,fillstyle=solid,fillcolor=curcolor]
{
\newpath
\moveto(389.03772726,684.23444145)
\lineto(386.90074458,691.1796635)
}
}
{
\newrgbcolor{curcolor}{0.98823529 0.10980392 0.98039216}
\pscustom[linewidth=0.99999871,linecolor=curcolor]
{
\newpath
\moveto(389.03772726,684.23444145)
\lineto(386.90074458,691.1796635)
}
}
{
\newrgbcolor{curcolor}{0.01176471 0.627451 0.2}
\pscustom[linewidth=0.99999871,linecolor=curcolor]
{
\newpath
\moveto(316.75968631,654.84109342)
\curveto(346.22572222,675.61840365)(410.60956978,689.66210759)(451.81227844,686.38484145)
\curveto(483.46449891,683.86722255)(498.16882647,662.0980131)(520.75516978,620.65296113)
\curveto(540.26263434,584.85754696)(545.12133041,533.57710602)(545.12133041,533.57710602)
\curveto(545.12133041,533.57710602)(533.16683592,505.8476194)(494.50022804,467.46746192)
\curveto(464.49474773,437.68425562)(402.70223119,415.14636586)(402.70223119,415.14636586)
\curveto(402.70223119,415.14636586)(359.50046615,422.35539893)(329.4149619,433.84595641)
\curveto(313.50133671,439.92385247)(278.07210206,456.87631861)(264.43862049,467.08966035)
\curveto(256.86784505,472.7612194)(247.84356537,479.96855169)(246.87233639,489.37810129)
\curveto(245.58803781,501.82075956)(250.34707151,561.0548005)(266.70523718,594.20911861)
\curveto(278.38752253,617.88649814)(278.97852726,628.20056428)(316.75968631,654.84109342)
\closepath
}
}
{
\newrgbcolor{curcolor}{1 0 0}
\pscustom[linestyle=none,fillstyle=solid,fillcolor=curcolor]
{
\newpath
\moveto(479.77184514,686.23478626)
\curveto(479.77184514,672.17591133)(468.13743913,660.77894135)(453.78567201,660.77894135)
\curveto(439.43390488,660.77894135)(427.79949887,672.17591133)(427.79949887,686.23478626)
\curveto(427.79949887,700.29366119)(439.43390488,711.69063117)(453.78567201,711.69063117)
\curveto(468.13743913,711.69063117)(479.77184514,700.29366119)(479.77184514,686.23478626)
\closepath
}
}
{
\newrgbcolor{curcolor}{1 0 0}
\pscustom[linestyle=none,fillstyle=solid,fillcolor=curcolor]
{
\newpath
\moveto(337.3767874,676.42371024)
\lineto(339.5137663,670.27986142)
\lineto(339.5137663,670.27986142)
}
}
\end{pspicture}

